On time and consistency in multi-level agent-based simulations

The integration of multiple viewpoints became an increasingly popular approach to deal with agent-based simulations. Despite their disparities, recent approaches successfully manage to run such multi-level simulations. Yet, are they doing it appropriately? This paper tries to answer that question, with an analysis based on a generic model of the temporal dynamics of multi-level simulations. This generic model is then used to build an orthogonal approach to multi-level simulation called SIMILAR. In this approach, most time-related issues are explicitly modeled, owing to an implementation-oriented approach based on the influence/reaction principle.

==> sections/acknowledgments.tex <==
%\section*{Acknowledgments}
The present research work has been supported by International Campus on 
Safety and Intermodality in Transportation (CISIT), the Nord-Pas-de-Calais 
Region, the European Community, the Regional Delegation for Research and 
Technology, the Ministry of Higher Education and Research, and the National 
Center for Scientific Research (CNRS). The authors gratefully acknowledge the 
support of these institutions.
Authors would also like to thank Hassane Aboua\"issa, Daniel Jolly and Jean-Baptiste Soyez for their help and support. 
